Efficient Deep Learning for Medical Imaging: Bridging the Gap Between High-Performance AI and Clinical Deployment

Deep learning has revolutionized medical image analysis, playing a vital role in modern clinical applications. However, the deployment of large-scale models in real-world clinical settings remains challenging due to high computational costs, latency constraints, and patient data privacy concerns associated with cloud-based processing. To address these bottlenecks, this review provides a comprehensive synthesis of efficient and lightweight deep learning architectures specifically tailored for the medical domain. We categorize the landscape of modern efficient models into three primary streams: Convolutional Neural Networks (CNNs), Lightweight Transformers, and emerging Linear Complexity Models. Furthermore, we examine key model compression strategies (including pruning, quantization, knowledge distillation, and low-rank factorization) and evaluate their efficacy in maintaining diagnostic performance while reducing hardware requirements. By identifying current limitations and discussing the transition toward on-device intelligence, this review serves as a roadmap for researchers and practitioners aiming to bridge the gap between high-performance AI and resource-constrained clinical environments.

==> tex/methodology.tex <==
\section{Research methodology} \label{sec:methodology}
This survey was conducted following a systematic review protocol to ensure comprehensive coverage of lightweight deep learning models in medical imaging. The methodology focuses on identifying architectures and optimization techniques specifically designed for resource-constrained environments and practical clinical deployment.

We performed a systematic literature search across major scientific databases, including IEEE Xplore, PubMed, Scopus, and Google Scholar/arXiv, covering the period from January 2020 to December 2025. To capture the diverse landscape of efficient AI, we constructed three distinct search queries targeting medical image analysis domains of lightweight modeling:

\begin{figure*}[ht]
    \centering
    \includegraphics[width=1.0\textwidth]{images/Graph.png}
    \caption{Number of publications over the years, categorized by architecture (CNNs, Transformers, SSMs)}
    \label{fig:graph}
\end{figure*}

\begin{itemize}[leftmargin=*]
    \item \textbf{Group 1: Lightweight Architectures (CNNs \& Transformers).} Targeted efficient backbone designs.
    \begin{quote}
        \texttt{(``Medical Image Analysis'' OR ``Medical Imaging'') AND (``Lightweight'' OR ``Efficient'' OR ``Compact'' OR ``Mobile'') AND ("Deep Learning" OR "CNN" OR "Transformer") AND ("Real-time" OR "On-device" OR "Edge")}
    \end{quote}
    
    \item \textbf{Group 2: Linear Complexity Models (SSMs).} Targeted emerging State Space Models and Mamba-based architectures.
    \begin{quote}
        \texttt{("Medical Imaging") AND ("Mamba" OR "State Space Model" OR "SSM" OR "VM-UNet" OR "MedMamba" OR "Vision Mamba" OR "Selective Scan")}
    \end{quote}
    
    \item \textbf{Group 3: Optimization \& Deployment.} Targeted model compression techniques and hardware-specific implementations.
    \begin{quote}
        \texttt{("Medical Imaging") AND ("Knowledge Distillation" OR "Quantization" OR "Pruning" OR "Teacher-Student") AND ("Deployment" OR "FPGA" OR "Embedded" OR "Mobile")}
    \end{quote}
\end{itemize}

To ensure the survey focuses on practical, deployment-ready solutions, strict eligibility criteria were applied. Papers were filtered based on the following rules:

\paragraph{Inclusion Criteria:}
\begin{enumerate}
    \item \textbf{Domain Relevance:} Studies must focus on 2D medical image analysis (e.g., X-ray, Ultrasound, Dermoscopy, or 2D slices of CT/MRI).
    \item \textbf{Task Relevance:} Priority is given to fundamental diagnostic tasks: Classification, Segmentation, and Detection.
    \item \textbf{Quantitative Reporting:} Articles must report specific efficiency metrics, including Number of Parameters (Params), Floating Point Operations (FLOPs), or Inference Speed (FPS/Latency), alongside standard performance metrics (Dice/Accuracy).
    \item \textbf{Novelty:} Papers proposing novel lightweight modules, architecture redesigns, or compression pipelines.
\end{enumerate}

\paragraph{Exclusion Criteria:}
\begin{enumerate}
    \item \textbf{Generative Tasks:} Studies focusing solely on Image Generation (GANs, Diffusion Models) or Reconstruction were excluded, as these are typically offline tasks not prioritized for real-time edge diagnostics.
    \item \textbf{Missing Metrics:} Papers that reported accuracy but failed to provide computational complexity metrics (Params/FLOPs) were excluded, as efficiency could not be verified.
\end{enumerate}


